Im4D: High-Fidelity and Real-Time Novel View Synthesis for Dynamic Scenes

This paper aims to tackle the challenge of dynamic view synthesis from multi-view videos. The key observation is that while previous grid-based methods offer consistent rendering, they fall short in capturing appearance details of a complex dynamic scene, a domain where multi-view image-based rendering methods demonstrate the opposite properties. To combine the best of two worlds, we introduce Im4D, a hybrid scene representation that consists of a grid-based geometry representation and a multi-view image-based appearance representation. Specifically, the dynamic geometry is encoded as a 4D density function composed of spatiotemporal feature planes and a small MLP network, which globally models the scene structure and facilitates the rendering consistency. We represent the scene appearance by the original multi-view videos and a network that learns to predict the color of a 3D point from image features, instead of memorizing detailed appearance totally with networks, thereby naturally making the learning of networks easier. Our method is evaluated on five dynamic view synthesis datasets including DyNeRF, ZJU-MoCap, NHR, DNA-Rendering and ENeRF-Outdoor datasets. The results show that Im4D exhibits state-of-the-art performance in rendering quality and can be trained efficiently, while realizing real-time rendering with a speed of 79.8 FPS for 512x512 images, on a single RTX 3090 GPU.

==> figures/teaser.tex <==
\begin{figure}
    \centering
    \vspace{-2.5mm}
    \includegraphics[width=0.9\linewidth]{figures/pdfs/teaser_final.pdf}
    \vspace{-2.5mm}
    \caption{\textbf{Rendering results on the DNA-Rendering \cite{renbody} dataset.} Our method produces high-fidelity rendering with high-quality depth results on a long dynamic scene with complex motions. All the rendered depths are normalized using the same method with the same hyperparameters and then combined with the rendered alpha map.
    ENeRF \cite{lin2022enerf} struggles to recover correct depth, leading to flicker and ghosting artifacts. K-Planes \cite{fridovich2023k} cannot recover the appearance details on this complex scene. Please refer to our supplementary video for better visualization. } 
    \label{fig:teaser}
    \vspace{-5mm}
\end{figure}


==> tables/ana_speed.tex <==
\begin{table}
    \tabcolsep=0.2cm
    \begin{center}
    \caption{\textbf{Analysis of rendering time.} 0 means that methods are tested with their officially released pre-trained model. The best and second-best results are highlighted \textfirst{green} and \secondtext{yellow}, respectively.}
    \label{tab:ana_speed}
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{l|c|ccc}
    \Xhline{3\arrayrulewidth}
    & Training time (hour) & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$  \\
    \Xhline{3\arrayrulewidth}
    \multirow{2}{*}{K-Planes} & 2   & 26.34  & 0.943 & 0.134  \\ 
     & 8 & 27.45 & 0.952  & 0.118  \\ \hline
    \multirow{2}{*}{IBRNet} & 0 & 25.31 & 0.954 & 0.106  \\
    & 3 & 27.85 & 0.967 & 0.081 \\ \hline
    \multirow{2}{*}{ENeRF} & 0 & 26.85 & 0.966 & 0.073 \\
    & 3 & \cellsecond 28.07 & \cellsecond 0.968 & \cellsecond 0.066 \\ \hline
    \multirow{3}{*}{Ours} & 0.51 & 27.14 & 0.961 & 0.083 \\
     & 3.33 &\cellfirst 28.99 &\cellfirst 0.973 & \cellfirst 0.062 \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    }
    \end{center}
    \vspace{-1em}
\end{table}


==> tables/supp_sport1.tex <==
\begin{table}
    \tabcolsep=0.1 cm
    \begin{center}
    \caption{\textbf{Quantitative ablation of view synthesis results on NHR and DNA-Rendering datasets.} Tt represents the training time, and its corresponding unit is hours. The detailed descriptions can be found in Sec. \ref{sec:ablation}.}
    \label{tab:ab_zju_nhr}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|ccc|ccc}
    \Xhline{3\arrayrulewidth}
     &  \multicolumn{3}{c|}{NHR} & \multicolumn{3}{c}{DNA-Rendering} \\
    % \hline
    %  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FPS  $\uparrow$ \\
      & PSNR $\uparrow$  & LPIPS $\downarrow$  & Tt $\downarrow$ & PSNR $\uparrow$  & LPIPS $\downarrow$  & Tt $\downarrow$ \\
    \hline
    1) Complete model & 34.87 & 0.043 & 2.29 & 29.82 & 0.045 & 3.33  \\
    2) w/o \textit{image-based} appearance &  31.79 & 0.107 & 1.81 & 26.07 & 0.102 & 2.54  \\
    3) w/o \textit{global} geometry     &  24.71 & 0.152 & 2.81 & 27.44 & 0.100 & 4.04  \\
    % 4) IBRNet     &  34.65 & 0.068 & 2.00 & 32.40 & 0.962  \\
    \hline
    4) $\numJointTraining = 0$, \quad\, $\numFinetuneTraining = \infty$ & 30.44 & 0.051 & 2.21 &  28.25 & 0.047 & 3.23 \\
    5) $\numJointTraining = 0$, \quad\, $\numFinetuneTraining = 20$  & 34.30 & 0.044 & 2.25 & 29.63 & 0.047 & 3.29 \\
    6) $\numJointTraining = 5000$, $\numFinetuneTraining = \infty$ & 34.29 & 0.043 & 2.26 & 29.27 & 0.045 & 3.27 \\
    7) $\numJointTraining = \infty$, \quad $\numFinetuneTraining = \textbackslash$ &34.89 & 0.042 & 3.19 & 29.83 & 0.045 & 4.55 \\ \hline
    8) w/o pre-trained model & 35.11& 0.042 & 2.29 & 29.58 & 0.047 & 3.33 \\  \hline
    9) \textit{inferring} ability & 34.82& 0.045 & 2.26 & 29.00 & 0.050 & 3.27 \\ 
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    }
    \end{center}
\end{table}
